Hierarchies of resources for measurement-based quantum computation

For certain restricted computational tasks, quantum mechanics provides a provable advantage over any possible classical implementation. Several of these results have been proven using the framework of measurement-based quantum computation (MBQC), where non-locality and more generally contextuality have been identified as necessary resources for certain quantum computations. Here, we consider the computational power of MBQC in more detail by refining its resource requirements, both on the allowed operations and the number of accessible qubits. More precisely, we identify which Boolean functions can be computed in non-adaptive MBQC, with local operations contained within a finite level in the Clifford hierarchy. Moreover, for non-adaptive MBQC restricted to certain subtheories such as stabiliser MBQC, we compute the minimal number of qubits required to compute a given Boolean function. Our results point towards hierarchies of resources that more sharply characterise the power of MBQC beyond the binary of contextuality vs non-contextuality.

==> drafts/SummaryOfResults.tex <==
For a temporally flat, non-contextual $l2$-MBQC, the only Boolean functions that can be computed with high probability are linear~\cite{Raussendorf2013}.\footnote{For qudits of prime dimension $d$, a similar result bounds the degree of computable functions to be less than $d$ \cite{FrembsRobertsBartlett2018,hoban2011generalized}.} This bound is not very sharp and there is room for a much finer characterisation. In particular the question of how to construct $l2$-MBQC schemes that compute general Boolean functions, as well as what resources besides contextuality, e.g. non-Clifford operations, qubits, time etc., are required in that case remains open. A better characterisation therefore seems an important milestone towards more practical realisations of the results in Ref.~\cite{BravyiGossetKoenig2018}.



\subsection{Completeness of temporally flat $l2$-MBQC}

We begin by recalling that temporally flat $l2$-MBQC is \textit{complete}, as characterised by the following theorem.

\begin{theorem}[\cite{HobanCampbell2011}]\label{thm: ld-MBQC universal}
	For any function $f: \zz_2^n \rightarrow \zz_2$ there exists a temporally flat $l2$-MBQC that deterministically evaluates $f$.%	Any function $o: \zz_d^n \rightarrow \zz_d$ can be computed within flat, deterministic $ld$-MBQC.
\end{theorem}


In other words, flat $l2$-MBQC can be arbitrarily contextual. We give an explicit proof of this theorem in Sec.~\ref{secCompleteness}, in order to show how resource states and measurement patterns are utilized. We also provide a generalisation to the qudit case for $d$ prime in App.~\ref{sec: Proof of lm: qudit delta function}, for which a similar contextuality threshold has been found in \cite{FrembsRobertsBartlett2018,hoban2011generalized}.
%In addition, we construct examples of MBQCs that compute functions violating the non-contextual bounds of Ref.~\cite{Raussendorf2013} and are thus contextual.

Note that the measurements operators in the MBQC constructed in the proof are \emph{non-Clifford}. Moreover, the MBQC is not \textit{efficient}, in that it requires (in general) $O(\exp(n))$ many qubits to compute $f$. In order to find a finer classification of this resource, a natural question thus is to ask for the optimality of such MBQCs in terms of non-Clifford resources and qubit count. We address these questions in the following sections.



\subsection{Temporally flat $l2$-MBQC and Clifford hierarchy}

The first restricted model of computation we consider is stabilizer MBQC -- where the resource states are stabilizer states and the operations are Clifford. In this case, the computable functions are heavily restricted. 

\begin{definition}
   We denote by $\Omega_n^2(\delta)$ the set of degree $\delta$ polynomials
\begin{equation}
    \Omega_n^2(\delta)
    %= \zz_2 \left[ \prod_{i = 1}^{n}x_i^{a_i} \mid a_i \in \zz_2, ~ \sum_{i=1}^{n} a_i \leq \delta\right]
    = \{f: \zz_2^n \rightarrow \zz_2 \mid \mathrm{deg}(f) \leq \delta\}\; .
\end{equation}
%where $\zz_2 [ \cdot ]$ denotes the $\zz_2$ linear span.
%\srob{[FIXME: drop $\zz$, $n$ is usually for number of qubits (as in Pauli group).]} \mf{Should we drop the notation $\Omega_n^2$ altogether and simply use $\zz_2[x_1,\cdots,x_n]$, maybe with a subscript $\delta$ to indicate the limitation on degree?}
\end{definition}
As an important instance, elements of $\Omega_n^2(2)$ are quadratic functions.

\begin{theorem}\label{thm:stabdeterm}
	For a temporally flat, stabilizer $l2$-MBQC with deterministic output, only quadratic functions can be computed.
\end{theorem}

In the more general non-deterministic case, we can bound the success probability in terms of the distance of the desired function to the nearest quadratic function. The success probability for an MBQC implementing a certain function is defined as follows.

\begin{definition}(Success probability)
	Consider a flat $l2$-MBQC aiming to compute a Boolean function $f: \zz_2^n \rightarrow \zz_2$. If a strategy succeeds with probability $p(\mathbf{i})$ on input string $\mathbf{i}$, then we define the overall success probability by $P_{succ}=\sum_{\mathbf{i} \in \zz^n_2} p(\mathbf{i})/2^n$.
\end{definition}


In the case that an $l2$-MBQC has deterministic output $g: \zz_2^n \rightarrow \zz_2$, the success probability reduces to $P_{succ}=1- d_H(f,g)/2^n$ where $d_H(\cdot, \cdot)$ denotes the Hamming distance between two functions (the number of inputs $\mathbf{i}$ where $f(\mathbf{i})\neq g(\mathbf{i})$) and $f: \zz_2^n \rightarrow \zz_2$ is the desired output function. Clearly, $P_{succ}=1$ if and only if $f=g$.

In order to compute the success probability for general functions, we consider the \emph{non-quadraticity} of a function, which measures how far a function is from being quadratic (see e.g.~\cite{Kolokotronis2007}):
\begin{equation}
\mathcal{NQ}(f) := \mathrm{min} \{ d_{H}(f,q) :  q \in \Omega_n^2(2) \} ,
\end{equation}
where again, $\Omega_n^2(2)$ denotes the set of quadratic Boolean functions over $n$ variables. Then we have the following characterisation of the computational power of temporally flat qubit stabilizer MBQC.


\begin{theorem}\label{thm: stabiliser success probability}
	Let $f: \zz_2^n \rightarrow \zz_2$ be an arbitrary Boolean function. The maximum success probability of computing this function in temporally flat, stabiliser MBQC is
	\begin{equation}
	P_{succ} \ =\ 1 - \frac{\mathcal{NQ}(f)}{2^k} .
	\end{equation}
\end{theorem}

Recall from Ref~\cite{Raussendorf2013} that any non-contextual qubit MBQC can only compute linear functions with high probability. We remark that despite the qubit stabilizer theory being contextual (\srob{[is there a clean quantitative measure for contextuality that can be used here?. Maybe just cite here or later in the discussion connections between contextuality/magic/negativity as a measure].}), temporally flat $l2$-MBQCs can only be lifted to being able to evaluate quadratic Boolean functions. This hints that there is a hierarchy of different strengths of contexuality correlations, with qubit stabilizer theory reaching only the lowest non-trivial step of the ladder.

In analogy to the stabilizer case, we can place a lower bound on the necessity of certain non-Clifford resources that are required to implement a general function in the temporally flat case. The following theorem shows that operations from the $D$'th level of the Clifford hierarchy are required whenever an $l2$-MBQC compute a polynomial of degree $D$.

\begin{theorem}\label{thm:CliffHierNec}
	For a temporally flat, deterministic $l2$-MBQC that belongs to level-$D$ of the Clifford hierarchy, only polynomials of degree at most $D$ can be computed.
\end{theorem}

This theorem can be viewed as a generalisation of Thm.~\ref{thm:stabdeterm}. 
One may naturally ask for the resource cost for both space (qubit count) and time required to implement a given function. As we will see in the next section, the problem of determining the minimal number of qubits in the temporally flat case is hard in general.

\subsection{Temporally flat $l2$-MBQC with a restriction on the qubit count}

Having seen (temporally flat) qubit stabilizer $l2$-MBQCs can only compute quadratic functions in the deterministic case, we begin by asking how many resources are required to do so. For a given function $o: \zz_2^n \rightarrow \zz_n$, let $R(o)$ denote the optimal number of resources required to implement it in $l2$-MBQC.

\begin{proposition}\label{prop: resource of quadratic Boolean functions}
	Let $f$ be a quadratic Boolean function of the form
	\begin{equation}
	f(x) = \sum_{i=1}^n l_i x_i + \sum_{i<j} q_{i,j} x_i x_j, \quad l_i, q_{i,j} \in \zz_2\; .
	\end{equation}
	Then $f$ can be computed deterministically within temporally flat, stabiliser $l2$-MBQC on $R(f) = \mathrm{rk}(f)+1$ qubits, where $\mathrm{rk}(f)$ is the $\zz_2$-rank of the symmetric matrix $Q(f)$ defined such that $Q_{i,i}=0$ and $Q_{i,j}=Q_{j,i}=q_{i,j}$. 
\end{proposition}
%\begin{proposition}
	%Let $f: \zz_2^n \rightarrow \zz_2$ be a quadratic Boolean function. Then $f$ can be computed within flat stabiliser $l2$-MBQC on $R(f) = \mathrm{rk}(f)+1$ qubits.
%\end{proposition}

%We give the proof in Sec.~\ref{SecGeneralResourceRequirements} and App.~\ref{sec: Proof of prop: resource of quadratic Boolean functions}.
Note that Prop.~\ref{prop: resource of quadratic Boolean functions} is independent of any resource state. As seen in the proof of Thm.~\ref{thm: ld-MBQC universal}, GHZ states are a universal resource for function computation.\footnote{Note however, that GHZ states are not universal for MBQC in general.} It is thus interesting to ask for the most qubit efficient MBQC, which achieves an arbitrary function, using the GHZ resource state
\begin{equation}\label{eq: N-qubit GHZ state}
    |\psi\rangle = \frac{1}{\sqrt{2}} (|0\rangle^{\otimes N} + |1\rangle^{\otimes N})\; .
\end{equation}
Let $\Omega_n^2$ be the space of functions $f:\zz_2^n\rightarrow \zz_2$, and let $\mathcal{F} \in \text{End}_{\mathbb{R}}(\Omega_n^2)$ be the linear Hadamard transform (defined explicitly in Sec.~\ref{sec: Polynomial vs Z_2-linear function representation} below). For any Boolean function $f \in \Omega_n^2$ we define the linear space of \emph{zero terms} as
\begin{equation}\label{eq: zero terms0}
Z(f) = \left\langle 2^m g \mid g: \zz_2^n \rightarrow \zz_2, n \geq m \geq 1 \right\rangle\; .
\end{equation} 
With this we can characterise the optimal number of resources $R(f)$ required to implement a given function $f: \zz_2^n \rightarrow \zz_n$ in $l2$-MBQC with a GHZ resource state as follows.

\begin{proposition}\label{prop: zero term reduction}
	The minimal number of qubits $R(f)$ required to deterministically implement a given polynomial function $f: \zz_2^n \rightarrow \zz_2$, in temporally flat $l2$-MBQC using GHZ states is the minimal number of non-zero coefficients $C_\mathbf{a}$ in $\mc{F}^{-1}(f)$ under the equivalence relation $f \sim f' \Longleftrightarrow f' = f + z$, $z \in Z(f)$ of Eq.~(\ref{eq: zero terms0}). 
\end{proposition}

Note that Prop.~\ref{prop: zero term reduction} only characterises $R$, yet does not provide a way to solve for it.



%Clearly, this replicates the Anders-Browne result as a special case, where $o(x)=x_1 x_{2}$ is a quadratic with
%\begin{equation}
%Q = \left( \begin{array}{cc} 0 & 1 \\
%1 & 0 \end{array}
%\right) .
%\end{equation}
%This is a rank 2 matrix and so the theorem says it can be computed using 3 qubits. We will study this resource aspect inherent to Prop.~\ref{prop: resource of quadratic Boolean functions} in more detail in Sec.~\ref{sec: Towards a classification of Boolean functions}.\\


While the stabilizer setting admits a simple characterisation, the correspondence between the degree of a Boolean function and the minimal number of qubits required for its implementation in flat $l2$-MBQC does not generalise easily. In fact, the general problem of computing qubit costs as defined in Prop.~\ref{prop: zero term reduction} is related to a problem in circuit synthesis (specifically minimum distance decoding of punctured Reed-Muller codes) which is known to be hard in general \cite{AmyMosca2016,seroussi1983maximum}. Nevertheless, using the above characterisation, we find the optimal qubit costs to compute the $n$-dimensional delta function in Sec.~\ref{SecGeneralResourceRequirements}, and we provide upper bounds on a family of functions known as elementary symmetric functions. As a consequence, we find that the number of qubits required to deterministically compute a function (with an $l2$-MBQC) is not monotonic in its degree (cf. Prop.~\ref{prop: mismatch degree vs qubit count}), thus hinting at a rich substructure of contextuality.\\



\subsection{Adaptivite $l2$-MBQC}
Finally, in the discussion and App.~\ref{secAdaptivity}, we briefly consider the role of adaptivity. We find that adaptive MBQCs -- that is, MBQCs where measurement outcomes are allowed to influence future measurement settings -- can have drastically reduced resource requirements to compute a given function. In particular, adaptive stabilizer MBQCs are functionally complete (they can compute arbitrary functions) in contrast to the temporally flat case where only quadratic functions may be computed. Additionally, space-time tradeoffs are possible, allowing for a much broader class of functions to be computed for a given qubit count.


%\srob{[We should discuss this section and maybe de-emphasize its role. It is currently example driven, and contained within the stabilizer formalism. It could use a statement about general computations, and could involve some canonical form for general computations (a canonical form consists of sequences of temporally flat "boxes" -- see for e.g. the chained AB boxes to produce a delta function. One could for instance use a greedy algorithm to optimise).]}

%\subsubsection{Space time trade-offs in stabilizer MBQC}
%We also consider adaptive MBQC. As originally observed by Anders and Browne, adaptivity is sufficient to lift stabilizer MBQC to functional completeness (i.e. any Boolean function can be evaluated by an adaptive qubit stabilizer MBQC)~\cite{AndersBrowne2009}. In the presence of adaptivity, we are therefore able to make tradeoffs between resources of space (i.e. qubits) and time, along with reducing the necessary non-Clifford resources. 

%The salient example here comes from the observation that the $n$-dimensional delta function $\delta : \zz_d^n \rightarrow \zz_d$
%\begin{align}\label{eq: n-dimensional delta function}
%\delta(\mathbf{i}) &:= \begin{cases} 1 &\mathrm{if\ } \mathbf{i}=\mathbf{0} \\ 0 &\mathrm{elsewhere.} \end{cases}
%\end{align}
%can be implemented in adaptive stabilizer MBQC with only $3$ qubits (i.e. independent of $n$). In contrast, for temporally flat MBQC we observe that $d^n-1$ qubits are required for its implementation, as well as gates from the $n$'th level of the Clifford Hierarchy. We give a more precise treatment of the tradeoffs that can be made using adpativity in Sec.~\ref{secAdaptivity}. 

%\srob{Can we show that contextuality grows w.r.t. some measure in order to compute higher degree polynomials in the stabilizer setting? Seems like composing together AB boxes is about as good as you can get.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{MBQC Preliminaries}
%\srob{Maybe we just roll this into the subsequent section}

%This section is a brief technical summary of how the output function in MBQC arises from the outcomes of local measurements on a resource state.


%\subsection{Local measurement outcomes and global computation output}
%\textcolor{blue}{\textbf{[include a brief description of local outcomes/phases combining to global output. The output function may be expressed in terms of polynomials over finite fields. Some results from App.~\ref{OldPhaseRelations}]}} 
